AER-LLM: Ambiguity-aware Emotion Recognition Leveraging Large Language Models

Recent advancements in Large Language Models (LLMs) have demonstrated great success in many Natural Language Processing (NLP) tasks. In addition to their cognitive intelligence, exploring their capabilities in emotional intelligence is also crucial, as it enables more natural and empathetic conversational AI. Recent studies have shown LLMs' capability in recognizing emotions, but they often focus on single emotion labels and overlook the complex and ambiguous nature of human emotions. This study is the first to address this gap by exploring the potential of LLMs in recognizing ambiguous emotions, leveraging their strong generalization capabilities and in-context learning. We design zero-shot and few-shot prompting and incorporate past dialogue as context information for ambiguous emotion recognition. Experiments conducted using three datasets indicate significant potential for LLMs in recognizing ambiguous emotions, and highlight the substantial benefits of including context information. Furthermore, our findings indicate that LLMs demonstrate a high degree of effectiveness in recognizing less ambiguous emotions and exhibit potential for identifying more ambiguous emotions, paralleling human perceptual capabilities.

==> 02-relatedwork.tex <==
\section{Related work}
Text-based emotion recognition has been explored for decades, with various feature sets and modeling frameworks examined. TF-IDF, which emphasizes frequent keywords to signal emotional cues, has been effectively employed in emotion classification~\cite{cahyani2021performance}. However, it fails to capture the meaning of sentences for effective emotion detection~\cite{alswaidan2020survey}. To address these issues, word embeddings have been proposed to capture semantic relationships in a dense representation. Pre-trained encoders such as Word2Vec, GloVe, and BERT are commonly used to extract word embeddings and have been fine-tuned to enhance emotion recognition~\cite{huang2019ana, agrawal2019nelec, bharti2022text}. %Huang employed a fine-tuned, pre-trained Bert model to achieve a better result in their classification tasks \cite{huang2019ana}.  
On the other hand, deep learning models have also been extensively studied for text-based emotion recognition. For instance, \cite{bharti2022text} proposed a hybrid model integrating Support Vector Machines (SVMs), Bi-Gated Recurrent Units (GRUs), and Convolutional Neural Networks (CNNs), achieving excellent results in text-based emotion recognition. Additionally, Contextual Emotion Detection (HRLCE) model leveraging the hierarchical Long Short-Term Memory (LSTM) networks was introduced in~\cite{huang2019ana}, which employs a multi-head self-attention mechanism to encode semantic and emotional information at the word level within each utterance.
However, effective feature extraction and classifers for emotion recognition generally require a large annotated dataset for training~\cite{bharti2022text, alswaidan2020survey}. 

More recently, the performance advances in Large Language Models (LLMs), such as LLAMA3~\cite{touvron2023llama} and GPT-4~\cite{achiam2023gpt}, have opened up new possibilities for text understanding and analysis. Their strong generalization capabilities enable effective text comprehension without the need for extensive retraining, such as through zero-shot or few-shot prompting~\cite{hu2024exploring}. 
One recent study proposed InstructERC~\cite{lei2023instructerc}, which treats emotion recognition in conversations as a retrieval-based Seq2Seq paradigm utilizing LLMs and present an instruction template suitable for various dialog scenarios. Additionally, it proposes multitasking by recognizing both speaker identity and emotions, thereby implicitly modeling dialogue role relationships to enhance emotional recognition.
 %The state-of-the-art InstructERC proposed by \cite{lei2023instructerc} significantly outperforms previous discriminant models by first identifying speakers and then conducting emotion prediction task using LLMs. 
Building on this, \cite{fu2024ckerc} further integrated a speaker commonsense identification task to better understand speaker characteristics, further enhancing performance in emotion recognition.

% the enhanced the InstructERC model by exploring implicit information about the speaker. The proposed model, called CKERC, is composed of a speaker commonsense identification task to better understand speaker characteristics and ERC tasks, resulting in competitive performance on popular datasets.

While LLMs show promise in emotion recognition, existing research has not addressed the inherent ambiguity of emotions, relying instead on majority vote annotations. For natural conversational AI, it is crucial to understand ambiguous emotions and their complexity to guide conversation flows similarly to humans. Although some studies account for ambiguity in emotions, they either use it as a loss function via KL divergence, ultimately aiming to recognize a single-label emotion \cite{zhou2022multi}, or treat ambiguous emotions as an out-of-distribution (OOD) separate class~\cite{wu2024handling}. None of these studies treat ambiguous emotions as a complete representation or develop models to capture this ambiguity, nor do they investigate LLMs' generative capabilities in understanding such ambiguous emotions. Especially leveraging in-context learning capabilities, LLMs can examine extended conversation histories to potentially improve the recognition of ambiguous emotions.

%A common approach is to embed KL divergence, a measure of similarity between two distributions, into the loss function of classifiers \cite{zhou2022multi,wu2024handling}. Specifically, \cite{zhou2022multi} proposed a multi-classifier interactive learning (MCIL) method, where different classifiers mimic how different people might interpret ambiguous emotion differently. In contrast, \cite{wu2024handling} groups utterances with ambiguous emotions into an additional class during the training of an emotion classifier. 

% \rev{Nevertheless, these studies either i) fail to fully capture emotional ambiguity through a distributional representation, treating it instead as an additional out-of-distribution (OOD) separate class, or ii) they heavily depend on hand-crafted features and traditional models, thereby not leveraging the potential of LLMs. Consequently, understanding the ambiguity of emotions through the capabilities of LLMs is important, which can pave the way for their future application in emotional conversational AI.}

% \cite{priyasad2020attention} study analyzed conversation using LSTM+Attention models for automatic emotion recognition. These studies only focus on single emotion categories. Recent studies have shifted to ambiguity-aware emotion recognition. \cite{wu2023distribution} proposed a distribution-based framework for ERC not only achieving a higher classification accuracy, but also demonstrating uncertainty estimation.  However, traditional models are deterministic and have limitations in handling long context, leading to poor generalization. Fortunately, LLMs can manage extended context without requiring additional training and can perform better by leveraging their pre-existing knowledge. \cite{lei2023instructerc} reformulated the ERC task and designed a retrieval module for LLMs which includes four components  (instruction, historical content, label statement and demonstration retrieval) to perform the emotion prediction task, while, their work did not address emotional ambiguity, which motivates the current study to explore this aspect further.  


% In our work, we will employ the Gemini Model, a LLM developed by Google and has achieved significant results in generative AI \cite{team2023gemini}, to design prompts and predict the probability distribution of emotions in a target sentence based on historical utterances. To assess Gemini's ability to understand ambiguous emotions, we evaluate its performance using majority-labeled agreement accuracy, alongside metrics such as Kullback Leibler (KL) divergence, Bhattacharyya Coefficient (BC), and R\textsuperscript{2} to measure the similarity between the ground truth and the predicted distributions.
% \td{can be combined with intro if less.}
% \td{check emotion recognition ambiguity paper; }

